Regularized Optimal Transport for Dynamic Semi-supervised Learning

Semi-supervised learning provides an effective paradigm for leveraging unlabeled data to improve a model's performance. Among the many strategies proposed, graph-based methods have shown excellent properties, in particular since they allow to solve directly the transductive tasks according to Vapnik's principle and they can be extended efficiently for inductive tasks. In this paper, we propose a novel approach for the transductive semi-supervised learning, using a complete bipartite edge-weighted graph. The proposed approach uses the regularized optimal transport between empirical measures defined on labelled and unlabelled data points in order to obtain an affinity matrix from the optimal transport plan. This matrix is further used to propagate labels through the vertices of the graph in an incremental process ensuring the certainty of the predictions by incorporating a certainty score based on Shannon's entropy. We also analyze the convergence of our approach and we derive an efficient way to extend it for out-of-sample data. Experimental analysis was used to compare the proposed approach with other label propagation algorithms on 12 benchmark datasets, for which we surpass state-of-the-art results. We release our code.

==> summary.tex <==
%\renewcommand*{\arraystretch}{1.2}
\setlength{\aboverulesep}{0pt}
\setlength{\belowrulesep}{0pt}
\setlength\LTleft{0pt}
\setlength\LTright{0pt}
\begin{longtable}{@{\extracolsep{\fill}}>{\footnotesize}c>{\footnotesize}c>{\footnotesize}c>{\footnotesize}c>{\footnotesize}c>{\footnotesize}c>{\footnotesize}c}
\caption{A summary of contributions presented in this survey for learning bounds in domain adaptation. \textbf{(Task)} refers to the considered learning problem; \textbf{(Framework)} specifies the statistical learning framework used in the analysis; \textbf{(Divergence)} is the metric used to compare the source and target distributions; \textbf{(Link)} stands for the dependence between the source error and the divergence term; \textbf{(Non-estim.)} indicates the presence of a non-estimable term in the bounds.} 
\endfirsthead
\endhead
\toprule
\addlinespace[.1cm]
\multirow{3}{*}{\footnotesize{\textbf{\textsc{Reference}}}}& \multicolumn{5}{c}{\footnotesize{\textbf{\textsc{Learning bounds}}}}\\
\addlinespace[.1cm]\cline{2-6}
\addlinespace[.1cm]
& \textbf{\textsc{Task}} & \textbf{\textsc{Framework}} & \textbf{\textsc{Divergence}} &	\textbf{\textsc{Link}} & \textbf{\textsc{Non-estim.}}\\
\addlinespace[.1cm]
\toprule
\addlinespace[.1cm]
\makecell{\cite{BenDavid07analysisof}\\\cite{Blitzer07Learning}\\\cite{bendavidth}} & \makecell{Binary\\ classification} & VC & $L^1$, $\hdh$ & Add. & $+$\\
\hline
\addlinespace[.1cm]
\cite{MansourMR09colt} & \makecell{Classification/\\ Regression} & Rademacher & Discrepancy & Add. & $+$\\
\addlinespace[.1cm]
\hline
\makecell{\cite{CortesMM10}\\\cite{CortesM14}\\\cite{CortesMM15}} & Regression & Rademacher & \makecell{(Generalized)\\ Discrepancy} & Add. & $+$\\
\hline
\addlinespace[.1cm]
\cite{KurokiCBHSS19} & \makecell{Classification} & Rademacher & (S-)Discrepancy & Add. & $+$\\
\addlinespace[.1cm]
\hline
\addlinespace[.1cm]
\cite{MansourMR08multiple} & \makecell{Classification/\\ Regression} & -- & -- & -- & --
\\
\addlinespace[.1cm]
\hline
\addlinespace[.1cm]
\makecell{\cite{MansourMR09}\\\cite{HoffmanMZ18}} & \makecell{Classification/\\ Regression} & -- & R\'enyi & Mult. & --\\
\addlinespace[.1cm]
\hline
\addlinespace[.1cm]
\cite{DhouibR18} & \makecell{Binary classification/\\Similarity learning} & -- & $L^1$, $\chi^2$ & Mult. & $+$\\
\addlinespace[.1cm]
\hline
\addlinespace[.1cm]
\cite{RedkoCFT19} & Binary classification & Rademacher & Discrepancy & Add. & $+$\\
\addlinespace[.1cm]
\hline
\addlinespace[.1cm]
\cite{ZhangZY12} & \makecell{Regression/ \\ Classification} & \makecell{Uniform \\entropy number} & IPM & Add. & --\\
\addlinespace[.1cm]
\hline
\addlinespace[.1cm]
\cite{Redko15} & Regression & Rademacher & IPM/MMD & Add. & $+$\\
\addlinespace[.1cm]
\hline
\addlinespace[.1cm]
\cite{RedkoHS16} & Regression & -- & IPM/Wassertein & Add. & $+$\\
\addlinespace[.1cm]
\hline
\addlinespace[.1cm]
\cite{zhang_bridging_2019} & \makecell{Large-margin\\classification} & Rademacher & IPM & Add. & $+$\\
\addlinespace[.1cm]
\hline
\addlinespace[.1cm]
\cite{JohanssonSR19} & \makecell{Classification} & -- & IPM & Add. & $+$\\
\addlinespace[.1cm]
\hline
\addlinespace[.1cm]
\cite{ShenQZY18} & Classification & -- & Wasserstein & Add. & $+$\\
\addlinespace[.1cm]
\hline
\addlinespace[.1cm]
\cite{CourtyFHR17} & Classification & -- & Wasserstein & Add. & $+$\\
\addlinespace[.1cm]
\hline
\addlinespace[.1cm]
\cite{pbda} & \makecell{Classification} & PAC-Bayes & Domain disagreement & Add. & $+$\\
\addlinespace[.1cm]
\hline
\addlinespace[.1cm]
\cite{dalc} & \makecell{Classification} & PAC-Bayes & $\beta$-divergence & Mult. & $+$\\
\addlinespace[.1cm]
\hline
\addlinespace[.1cm]
\cite{li2007bayesian} & Classification & PAC-Bayes & -- & Add. & --\\
\addlinespace[.1cm]
\hline
\addlinespace[.1cm]
\cite{McNamaraB17} & \makecell{Binary classification} & VC/PAC-Bayes & -- & Add. & --\\
\addlinespace[.1cm]
\hline
\addlinespace[.1cm]
\cite{MansourS14} & Classification & Robustness & $\lambda$-shift & Add. & --\\
\addlinespace[.1cm]
\hline
\addlinespace[.05cm]
\makecell{\cite{KuzborskijO13}\\\cite{KuzborskijO17}\\\cite{simonHTL}} & Regression & Stability & -- & -- & --\\
\addlinespace[.05cm]
\hline
\addlinespace[.1cm]
\cite{PerrotH15ICML} & \makecell{Classification/\\Similarity learning} & Stability & -- & -- & --\\
\addlinespace[.1cm]
\hline
\addlinespace[.1cm]
\cite{MorvantKAIS12} & \makecell{Classification/\\Similarity learning} & Robustness/VC & $\hdh$ & Add. & +\\
\addlinespace[.1cm]
\bottomrule
\end{longtable}
\begin{longtable}{@{\extracolsep{\fill}}>{\footnotesize}c>{\footnotesize}c>{\footnotesize}c>{\footnotesize}c>{\footnotesize}c>{\footnotesize}c>{\footnotesize}c}
\caption{A summary of contributions presented in this survey for hardness results in domain adaptation. \textbf{(Type)} is the type of the obtained result; \textbf{(Setting)} points out the presence or absence of target data (either labelled or unlabelled); \textbf{(Assumptions)} indicate the considered assumptions (individual or combined); \textbf{(Proper)} specifies if the learned model is required to belong to a predefined class; \textbf{(Constr.)} indicates if the result is of a constructive nature.} 
\endfirsthead
\endhead
\toprule
\addlinespace[.1cm]
\multirow{3}{*}{\footnotesize{\textbf{\textsc{Reference}}}}& \multicolumn{5}{c}{\footnotesize{\textbf{\textsc{Hardness results}}}}\\
\addlinespace[.1cm]\cline{2-6}
\addlinespace[.1cm]
& \textbf{\textsc{Type}} & \textbf{\textsc{Setting}} & \textbf{\textsc{Assumptions}} &	\textbf{\textsc{Proper}} & \textbf{\textsc{Constr.}}\\
\addlinespace[.1cm]
\toprule
\addlinespace[.1cm]
\cite{BenDavidLLP10} & \makecell{Impossibility/\\Sample compl.} & Unlabelled target & \makecell{Cov. shift,\\$\hdh$, $\lambda_\Hcal$} & -- & $+$\\
\addlinespace[.1cm]
\hline
\addlinespace[.1cm]
\cite{BenDavidSU12} & \makecell{Impossibility/\\Sample compl.} & \makecell{No target/\\Unlabelled target} & \makecell{Cov. shift,\\$C_{\cal B}$, Lipscht.} & $+$ & $+$/--\\
\addlinespace[.1cm]
\hline
\addlinespace[.1cm]
\cite{BenDavidU12} & \makecell{Impossibility/\\Sample compl.} & \makecell{Unlabelled target} & \makecell{Cov. shift,\\$C_{\cal B}$, Realizab.} & -- & --\\
\addlinespace[.1cm]
\hline
\addlinespace[.1cm]
\cite{RedkoHS19} & \makecell{Estimation/\\Sample compl.} & \makecell{Labelled target} & -- & -- & --\\
\addlinespace[.1cm]
\hline
\addlinespace[.1cm]
\cite{CZG19} & \makecell{Impossibility} & \makecell{Unlabelled target} & \makecell{Cov. shift,\\$\hdh$, $\lambda_\Hcal$} & -- & $+$\\
\addlinespace[.1cm]
\hline
\addlinespace[.1cm]
\cite{JohanssonSR19} & \makecell{Impossibility} & \makecell{Unlabelled target} & \makecell{Cov. shift,\\$\hdh$, $\lambda_\Hcal$} & -- & $+$\\
\addlinespace[.1cm]
\hline
\addlinespace[.1cm]
\cite{hanneke19} & \makecell{Sample compl.} & \makecell{Labelled target} & \makecell{Relaxed cov. shift,\\Noise cond.} & -- & --\\
\bottomrule
\end{longtable}
%
